When a language model is optimized for reasoning, does it still show embers of autoregression? An analysis of OpenAI o1

In "Embers of Autoregression" (McCoy et al., 2023), we showed that several large language models (LLMs) have some important limitations that are attributable to their origins in next-word prediction. Here we investigate whether these issues persist with o1, a new system from OpenAI that differs from previous LLMs in that it is optimized for reasoning. We find that o1 substantially outperforms previous LLMs in many cases, with particularly large improvements on rare variants of common tasks (e.g., forming acronyms from the second letter of each word in a list, rather than the first letter). Despite these quantitative improvements, however, o1 still displays the same qualitative trends that we observed in previous systems. Specifically, o1 -- like previous LLMs -- is sensitive to the probability of examples and tasks, performing better and requiring fewer "thinking tokens" in high-probability settings than in low-probability ones. These results show that optimizing a language model for reasoning can mitigate but might not fully overcome the language model's probability sensitivity.

==> deleted.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{figures/embers_0924_sorting_hard.pdf}
    \hspace{1cm}
    \includegraphics[scale=0.6]{figures/embers_decoding_shift_hard.pdf}
    \caption{Left: On datasets based on challenging sorting tasks, o1 performs better on the common type of sorting (i.e., sorting into alphabetical order) than on the rare type of sorting (i.e., sorting into reverse alphabetical order). Right: When decoding shift ciphers, o1 shows roughly the same performance on the common cipher type and on the rare cipher type when the examples are ones with a high output probability. However, when it is instead evaluated on examples with medium or low probability, its accuracy is higher for the common cipher type than the rare one. The error intervals in both plots indicate one standard error.}
    \label{fig:hardtasks}
\end{figure*}


